Mass and Eccentricity Constraints in the WASP-47 Planetary System from a Simultaneous Analysis of Radial Velocities & Transit Timing Variations

Measuring precise planet masses, densities, and orbital dynamics in individual planetary systems is an important pathway toward understanding planet formation. The WASP-47 system has an unusual architecture that motivates a complex formation theory. The system includes a hot Jupiter ("b") neighbored by interior ("e") and exterior ("d") sub-Neptunes, and a long-period eccentric giant planet ("c"). We simultaneously modeled transit times from the Kepler K2 Mission and 118 radial velocities to determine precise masses, densities, and Keplerian orbital elements of the WASP-47 planets. Combining RVs and TTVs provides a better estimate of the mass of planet d (13.6\pm2.0~M_\odot) than obtained with only RVs ($12.75\pm2.70~M_\odot$) or TTVs ($16.1\pm3.8~M_\odot$). Planets e and d have high densities for their size, consistent with a history of photo-evaporation and/or formation in a volatile-poor environment. Through our RV and TTV analysis, we find that the planetary orbits have eccentricities similar to the solar system planets. The WASP-47 system has three similarities to our own solar system: (1) the planetary orbits are nearly circular and coplanar, (2) the planets are not trapped in mean motion resonances, and (3) the planets have diverse compositions. None of the current single-process exoplanet formation theories adequately reproduce these three characteristics of the WASP-47 system (or our solar system). We propose that WASP-47, like the solar system, formed in two stages: first, the giant planets formed in a gas-rich disk and migrated to their present locations, and second, the high-density sub-Neptunes formed in situ in a gas-poor environment.

==> katdeck.tex <==
\section{First-Order Analytics of the Transit Timing Variations}
For two planets near first order ($j:j-1$) mean motion resonance \cite{Lithwick12b}, give the following expression for $V$ and $V^\prime$, the  complex TTV amplitudes of the inner and outer planets respectively.

\begin{align}
    V        & = P \frac{\mu^\prime}{\pi j^{2/3} (j - 1)^{1/3} \Delta } 
                 \left(-f  - \frac{3}{2}\frac{\Zfreestar}{\Delta}\right) \label{eqn:v} \\
    V^\prime & = P^\prime \frac{\mu}{\pi j \Delta } 
                 \left(-g  + \frac{3}{2}\frac{\Zfreestar}{\Delta}\right) \label{eqn:vprime}, 
\end{align}
where $V$ is the complex TTV amplitude, $P$ is the average orbital period, $\Delta$ is the normalized distance to resonance given by

\begin{equation}
    \Delta = \frac{P^\prime}{P}\frac{j-1}{j} -1
\end{equation}    
and \Zfree is a linear combination of the free complex eccentricities of the the two planets given by
\begin{equation}
\Zfree = f \zfree + g \zfreeprime
\end{equation}
and $f$ and $g$ are order sums of Laplace coefficients. \Zfreestar is the complex conjugate of \Zfree.

For WASP-47, $P = P_b = 4.1592$~d, $P^{\prime} = P_d = 9.0316$~d, $\Delta = 0.0857$, $f = -1.010$, $g_{\mathrm{ext}} = 0.4284 - 1.17\Delta = 0.328 $. We consider a useful limiting case where $\Zfree / \Delta \ll g $ and $f$. Detailed TTV analysis by \cite{Becker2015} found that

\begin{align*}
    e_d \cos \omega_d - e_b \cos \omega_b & = -0.0002\pm 0.0195 \\
                                          & \approx Re(\Zfree)\\
    e_d \sin \omega_d - e_b \sin \omega_b & = 0.0039\pm 0.0179\\
                                          & \approx Im(\Zfree).
\end{align*}
Therefore, for WASP-47, $\Zfree / \Delta \lesssim g $ and $f$. Taking this limit, dividing Equation~\ref{eqn:v} by Equation~\ref{eqn:vprime}, and rearranging terms, we find:

\begin{align}
\frac{M_d}{M_b} & = \frac{g}{f}\left(\frac{j-1}{j}\right)^{1/3} \frac{P_d}{P_b} \frac{|V_b|}{|V_d|}\\
                   & \approx \frac{ 0.112}{0.328}
                     \left(\frac{1}{2}\right)^{1/3} 
                     \left( \frac{9.031\ \mathrm{d}}{4.159\ \mathrm{d}}\right)
                     \left( \frac{0.75\ \mathrm{min}}{7.5\ \mathrm{min}}\right) \\
                   & \approx 0.056
\end{align}
The \cite{Lithwick12b} formula loses accuracy as one moves away from first order MMR (as noted in \citet{Lithwick12b} and \citet{DeckAgol2015}). This is because further away from resonance additional terms in the TTVs become comparable to the dominant terms associated with the resonance. For this system, with a period ratio of 2.17, these extra terms should be included. Using Equations (10)-(15) of Deck \& Agol 2015, the expression for the TTV amplitudes can be written as:
\begin{align}
    V &= {P \over 2\pi} \mu' f_1^{(2)}(\alpha) \nonumber \\
    V' & = {P' \over 2\pi} \mu f_2^{(1)}(\alpha)
\end{align}
where
\begin{align}
    \alpha & = \frac{a}{a'}, \nonumber \\
    f_1^{(2)}(\alpha) &= \alpha \frac{2 \beta D_\alpha b_{1/2}^{2}(\alpha)+(6+2\beta^2) b_{1/2}^{2}(\alpha) }{\beta^2 (1-\beta^2)},\\
    f_2^{(1)}(\alpha) &=  \bigg[(\kappa^2+3) b_{1/2}^{1}(\alpha)+2 \kappa (D_\alpha b_{1/2}^{1}(\alpha)+b_{1/2}^{1}(\alpha))\\
    &\qquad -\alpha^{-2} (\kappa^2-2\kappa+3) \bigg] \times \frac{1}{\kappa^2 (\kappa^2-1)},\\
    \beta &= 2(n-n')/n, \nonumber\\
    \kappa & = (n-n')/n',
\end{align}
and $D_\alpha$ is the derivative operator $\alpha \frac{\partial}{\partial \alpha}$, $n$ and $n'$ are the mean motions of the two planets, and $b_{1/2}^j(\alpha)$ is the usual Laplace coefficient.For the outer two planets in the Wasp-47 system, $\alpha = 0.596$, $f_1^{2} = -13.5$, and $f_2^{1} = 2.49$ (they are opposite in sign as the TTVs are anticorrelated).

We use a zeroth order formulae because we are considering the case where eccentricity effects are negligible, as argued above. In applying the formulae, we only include terms that would contribute a signal to the TTVs with a period equal to the ``super-period" of the 2:1 near resonance, as those are the signal amplitudes we are measuring from the TTVs.
Evaluating these TTV expressions, using TTV amplitudes of 7.5 min and 0.75 min, we find  $M_d / M_b \approx 0.040$. 

Note that in the limit where eccentricity contributions are negligible, these formulae can be used to estimate the masses directly, and not just the mass ratio of the two planets. By doing so we find that $\mu' = 5.83\times10^{-5}$ and $\mu = 1.46\times10^{-3}$ (again using measured amplitudes of 7.5 and 0.75 minutes). Given a stellar mass of $\sim M_\odot$, this yields planet masses of 19.4 $M_\oplus$ and 487 $M_\oplus$. {\bf not sure if you want to include this. but we can get the masses really simply from the formulae so might as well? That these are a bit high suggests that 0.75 and 7.5 min are too high as amplitudes. If I use Becker's measured TTV amplitude of 0.63 min, I get 16.3 earth masses. The HJ still has a mass that is too large, though. } 


